The effect of Target Normalization and Momentum on Dying ReLU

Optimizing parameters with momentum, normalizing data values, and using rectified linear units (ReLUs) are popular choices in neural network (NN) regression. Although ReLUs are popular, they can collapse to a constant function and "die", effectively removing their contribution from the model. While some mitigations are known, the underlying reasons of ReLUs dying during optimization are currently poorly understood. In this paper, we consider the effects of target normalization and momentum on dying ReLUs. We find empirically that unit variance targets are well motivated and that ReLUs die more easily, when target variance approaches zero. To further investigate this matter, we analyze a discrete-time linear autonomous system, and show theoretically how this relates to a model with a single ReLU and how common properties can result in dying ReLU. We also analyze the gradients of a single-ReLU model to identify saddle points and regions corresponding to dying ReLU and how parameters evolve into these regions when momentum is used. Finally, we show empirically that this problem persist, and is aggravated, for deeper models including residual networks.

==> empirical.tex <==
% !TEX root = main.tex
\section{Illustrating example}
\label{sec:empirical}

Before our analytic investigation in Sec. \ref{sec:affine} and
\ref{sec:single_relu}, we present a set of numerical examples that show the
effect of target normalization and momentum on regression in practice. Our model
is a shallow NN with ReLU activations that is optimized with Adam \citep{adam}.
For training data, we use four datasets from the UCI Machine Learning Repository
\citep{uci} all with single-variate target values,
which are normalized as described in Sec. \ref{sec:preliminaries}. For details
about the experiments,
see Appendix \ref{regression_details}.

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.49\textwidth]{figures/scale_bias_mse}
    \caption{
Effect of target normalization with scale $\gamma$ and bias $\delta$ on training MSE (left: $\delta = 0$, right: $\gamma = 1$). Shaded region shows $\pm$ the standard error of mean. For $\gamma = 1$ and $\delta = 0$, which is the common choice of zero mean and unit variance, a ``sweet spot'' can be observed.}
    \label{fig:scale_bias_rmse}
%    \todo{What is the value of the non-changing variable in the respective plots? Can you create a 3d plot, e.g. with color being the MSE? No 3d plot since the other variable is kept fixed. This is now explained.}
   % \todo{Can you make a 3d plot for the appendix? I.e. some sort of grid search and visualizing the height field with lines?}
%\end{figure}
%
%\begin{figure}[]
    \centering
    \includegraphics[width=0.49\textwidth]{figures/scale_dying}
    \caption{
  Effect of target normalization with scale $\gamma$ and bias $b = 0$.
  Decreasing $\gamma$ leads to more dying ReLUs when using Adam and eventually
  only few or no ReLUs output non-zero values. For SGD this effect is not observed. For
  large $\gamma$ and SGD, the training was very unstable, often resulting in
  nan-values. This portion of the SGD plot is therefore removed.}
    \label{fig:scale_dying}
\end{figure}

MSE results for Adam from several runs are show in \figref{fig:scale_bias_rmse},
where the errors are computed on target values using the same normalization for
comparability. It can be seen that the values of $\gamma$ and $\delta$ have an
important role in acheiving lower MSE scores. We also observe that the common
practice of setting $\gamma = 1$ and $\delta =0$ performs well in all instances
and therefore is an \emph{empirically} well motivated choice. To get an
understanding of why this is happening, we monitored the number of dead ReLU,
as shown in \figref{fig:scale_dying}. We observe that as target variances
($\gamma$) become smaller, the NN eventually entirely collapse to a constant
function. We also observe that this does not happen when instead using
stochastic gradient descent without momentum.

From these experiments,
we draw the conclusion that the deteriorating performance for $\gamma<1$ likely
is caused by dying ReLUs, although we do not claim it is the only reason.
We further conclude that ReLUs die as
a consequence of small target variances and the momentum-based optimizer Adam.
In the following sections, we investigate this
relationship more closely.

%We believe that the deterioration of how well the model fits the data is a
%complex problem that does not have a single simple explanation. That said
%we will in this paper focus our attention on dying
%ReLU in particular.

%\todo{
%  2) How can we make the connection to the following sections stronger (which at
%  the same time justifies why this example is presented)?
%}

